An Empirical Study of Software Exceptions in the Field using Search Logs

Software engineers spend a substantial amount of time using Web search to accomplish software engineering tasks. Such search tasks include finding code snippets, API documentation, seeking help with debugging, etc. While debugging a bug or crash, one of the common practices of software engineers is to search for information about the associated error or exception traces on the internet. In this paper, we analyze query logs from a leading commercial general-purpose search engine (GPSE) such as Google, Yahoo! or Bing to carry out a large scale study of software exceptions. To the best of our knowledge, this is the first large scale study to analyze how Web search is used to find information about exceptions. We analyzed about 1 million exception related search queries from a random sample of 5 billion web search queries. To extract exceptions from unstructured query text, we built a novel and high-performance machine learning model with a F1-score of 0.82. Using the machine learning model, we extracted exceptions from raw queries and performed popularity, effort, success, query characteristic and web domain analysis. We also performed programming language-specific analysis to give a better view of the exception search behavior. These techniques can help improve existing methods, documentation and tools for exception analysis and prediction. Further, similar techniques can be applied for APIs, frameworks, etc.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> paper_bbl <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{72}

%%% ====================================================================
%%% NOTE TO THE USER: you can override these defaults by providing
%%% customized versions of any of these macros before the \bibliography
%%% command.  Each of them MUST provide its own final punctuation,
%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
%%% do not use final punctuation, in order to avoid confusing it with
%%% the Web address.
%%%
%%% To suppress output of a particular field, define its macro to expand
%%% to an empty string, or better, \unskip, like this:
%%%
%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
%%%
%%% \def \showDOI #1{\unskip}           % plain TeX syntax
%%%
%%% ====================================================================

\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
\ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
\ifx \showURL      \undefined \def \showURL       {\relax}        \fi
% The following commands are used for tagged output and should be
% invisible to TeX
\providecommand\bibfield[2]{#2}
\providecommand\bibinfo[2]{#2}
\providecommand\natexlab[1]{#1}
\providecommand\showeprint[2][]{arXiv:#2}

\bibitem[\protect\citeauthoryear{??}{cas}{2010}]%
        {castillo2010}
 \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{The effects of query bursts on web search}. In
  \bibinfo{booktitle}{\emph{Proceedings - 2010 IEEE/WIC/ACM International
  Conference on Web Intelligence, WI 2010}}, Vol.~\bibinfo{volume}{1}.
  \bibinfo{pages}{374--381}.
\newblock
\showISBNx{9780769541914}
\urldef\tempurl%
\url{https://doi.org/10.1109/WI-IAT.2010.59}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{??}{csh}{2019}]%
        {csharpceptions}
 \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{CSharp Exception List}.
\newblock
  \bibinfo{howpublished}{\url{https://powershellexplained.com/2017-04-07-all-dotnet-exception-list/}}.
\newblock
\newblock
\shownote{Accessed: 2019-06-20.}


\bibitem[\protect\citeauthoryear{??}{jav}{2019}]%
        {javaexceptions}
 \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{Java Exception List}.
\newblock
  \bibinfo{howpublished}{\url{https://programming.guide/java/list-of-java-exceptions.html}}.
\newblock
\newblock
\shownote{Accessed: 2019-06-20.}


\bibitem[\protect\citeauthoryear{??}{par}{2019}]%
        {parserator}
 \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{Parserator}.
\newblock \bibinfo{howpublished}{\url{https://parserator.datamade.us/}}.
\newblock
\newblock
\shownote{Accessed: 2019-06-20.}


\bibitem[\protect\citeauthoryear{??}{pyt}{2019}]%
        {pythonexceptions}
 \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{Python Exception List}.
\newblock
  \bibinfo{howpublished}{\url{https://docs.python.org/3/library/exceptions.html}}.
\newblock
\newblock
\shownote{Accessed: 2019-06-20.}


\bibitem[\protect\citeauthoryear{??}{kru}{2020}]%
        {krugle}
 \bibinfo{year}{2020}\natexlab{}.
\newblock \bibinfo{title}{Krugle}.
\newblock \bibinfo{howpublished}{\url{https://www.krugle.com/}}.
\newblock
\newblock
\shownote{Accessed: 2020-04-30.}


\bibitem[\protect\citeauthoryear{Ai, Dumais, Craswell, and Liebling}{Ai
  et~al\mbox{.}}{2017}]%
        {QAi2017}
\bibfield{author}{\bibinfo{person}{Qingyao Ai}, \bibinfo{person}{Susan~T.
  Dumais}, \bibinfo{person}{Nick Craswell}, {and} \bibinfo{person}{Dan
  Liebling}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Characterizing Email Search Using Large-Scale
  Behavioral Logs and Surveys}. In \bibinfo{booktitle}{\emph{Proceedings of the
  26th International Conference on World Wide Web}} (Perth, Australia)
  \emph{(\bibinfo{series}{WWW ’17})}. \bibinfo{publisher}{International World
  Wide Web Conferences Steering Committee}, \bibinfo{address}{Republic and
  Canton of Geneva, CHE}, \bibinfo{pages}{1511–1520}.
\newblock
\showISBNx{9781450349130}
\urldef\tempurl%
\url{https://doi.org/10.1145/3038912.3052615}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Azzopardi, Kelly, and Brennan}{Azzopardi
  et~al\mbox{.}}{2013}]%
        {akb13-sigir}
\bibfield{author}{\bibinfo{person}{L. Azzopardi}, \bibinfo{person}{D. Kelly},
  {and} \bibinfo{person}{K. Brennan}.} \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{How Query Cost Affects Search Behavior}.
  \bibinfo{pages}{23--32}.
\newblock


\bibitem[\protect\citeauthoryear{Azzopardi, White, Thomas, and
  Craswell}{Azzopardi et~al\mbox{.}}{2020}]%
        {Azzopardi2020}
\bibfield{author}{\bibinfo{person}{Leif Azzopardi}, \bibinfo{person}{Ryen~W.
  White}, \bibinfo{person}{Paul Thomas}, {and} \bibinfo{person}{Nick
  Craswell}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Data-Driven Evaluation Metrics for Heterogeneous
  Search Engine Result Pages}. In \bibinfo{booktitle}{\emph{Proceedings of the
  2020 Conference on Human Information Interaction and Retrieval}} (Vancouver
  BC, Canada) \emph{(\bibinfo{series}{CHIIR ’20})}.
  \bibinfo{publisher}{Association for Computing Machinery},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{213–222}.
\newblock
\showISBNx{9781450368926}
\urldef\tempurl%
\url{https://doi.org/10.1145/3343413.3377959}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Bajracharya, Ngo, Linstead, Dou, Rigor, Baldi,
  and Lopes}{Bajracharya et~al\mbox{.}}{2006}]%
        {bajracharya2006sourcerer}
\bibfield{author}{\bibinfo{person}{Sushil Bajracharya}, \bibinfo{person}{Trung
  Ngo}, \bibinfo{person}{Erik Linstead}, \bibinfo{person}{Yimeng Dou},
  \bibinfo{person}{Paul Rigor}, \bibinfo{person}{Pierre Baldi}, {and}
  \bibinfo{person}{Cristina Lopes}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Sourcerer: a search engine for open source code
  supporting structure-based search}. In \bibinfo{booktitle}{\emph{Companion to
  the 21st ACM SIGPLAN symposium on Object-oriented programming systems,
  languages, and applications}}. ACM, \bibinfo{pages}{681--682}.
\newblock


\bibitem[\protect\citeauthoryear{Bajracharya and Lopes}{Bajracharya and
  Lopes}{2012}]%
        {Bajracharya2012}
\bibfield{author}{\bibinfo{person}{Sushil~Krishna Bajracharya} {and}
  \bibinfo{person}{Cristina~Videira Lopes}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{Analyzing and mining a code search engine usage
  log}.
\newblock \bibinfo{journal}{\emph{Empirical Software Engineering}}
  \bibinfo{volume}{17}, \bibinfo{number}{4} (\bibinfo{date}{01 Aug}
  \bibinfo{year}{2012}), \bibinfo{pages}{424--466}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1007/s10664-010-9144-6}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Bansal, Deligiannis, Maddila, and Rao}{Bansal
  et~al\mbox{.}}{2020}]%
        {bansal2020studying}
\bibfield{author}{\bibinfo{person}{Chetan Bansal}, \bibinfo{person}{Pantazis
  Deligiannis}, \bibinfo{person}{Chandra Maddila}, {and}
  \bibinfo{person}{Nikitha Rao}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \showarticletitle{Studying Ransomware Attacks Using Web Search Logs}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2005.00517}}
  (\bibinfo{year}{2020}).
\newblock


\bibitem[\protect\citeauthoryear{Bansal, Zimmermann, Awadallah, and
  Nagappan}{Bansal et~al\mbox{.}}{2019}]%
        {bansal2019usage}
\bibfield{author}{\bibinfo{person}{Chetan Bansal}, \bibinfo{person}{Thomas
  Zimmermann}, \bibinfo{person}{Ahmed~Hassan Awadallah}, {and}
  \bibinfo{person}{Nachiappan Nagappan}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{The Usage of Web Search for Software Engineering}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1912.09519}}
  (\bibinfo{year}{2019}).
\newblock


\bibitem[\protect\citeauthoryear{Carlson, Gaffney, and Vasile}{Carlson
  et~al\mbox{.}}{2009}]%
        {carlson2009learning}
\bibfield{author}{\bibinfo{person}{Andrew Carlson}, \bibinfo{person}{Scott
  Gaffney}, {and} \bibinfo{person}{Flavian Vasile}.}
  \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{Learning a Named Entity Tagger from Gazetteers with
  the Partial Perceptron.}. In \bibinfo{booktitle}{\emph{AAAI Spring Symposium:
  Learning by Reading and Learning to Read}}. \bibinfo{pages}{7--13}.
\newblock


\bibitem[\protect\citeauthoryear{Chancellor and Counts}{Chancellor and
  Counts}{2018}]%
        {chancellor2018measuring}
\bibfield{author}{\bibinfo{person}{Stevie Chancellor} {and}
  \bibinfo{person}{Scott Counts}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Measuring employment demand using internet search
  data}. In \bibinfo{booktitle}{\emph{Proceedings of the 2018 CHI Conference on
  Human Factors in Computing Systems}}. ACM, \bibinfo{pages}{122}.
\newblock


\bibitem[\protect\citeauthoryear{Chen, Lee, Xie, Yang, Lasecki, and Oney}{Chen
  et~al\mbox{.}}{2017}]%
        {Chen2017}
\bibfield{author}{\bibinfo{person}{Yan Chen}, \bibinfo{person}{Sang~Won Lee},
  \bibinfo{person}{Yin Xie}, \bibinfo{person}{YiWei Yang},
  \bibinfo{person}{Walter~S. Lasecki}, {and} \bibinfo{person}{Steve Oney}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Codeon: On-Demand Software Development Assistance}.
  In \bibinfo{booktitle}{\emph{Proceedings of the 2017 CHI Conference on Human
  Factors in Computing Systems}} (Denver, Colorado, USA)
  \emph{(\bibinfo{series}{CHI ’17})}. \bibinfo{publisher}{Association for
  Computing Machinery}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{6220–6231}.
\newblock
\showISBNx{9781450346559}
\urldef\tempurl%
\url{https://doi.org/10.1145/3025453.3025972}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Collier, Nobata, and Tsujii}{Collier
  et~al\mbox{.}}{2000}]%
        {collier2000extracting}
\bibfield{author}{\bibinfo{person}{Nigel Collier}, \bibinfo{person}{Chikashi
  Nobata}, {and} \bibinfo{person}{Jun-ichi Tsujii}.}
  \bibinfo{year}{2000}\natexlab{}.
\newblock \showarticletitle{Extracting the names of genes and gene products
  with a hidden Markov model}. In \bibinfo{booktitle}{\emph{Proceedings of the
  18th conference on Computational linguistics-Volume 1}}. Association for
  Computational Linguistics, \bibinfo{pages}{201--207}.
\newblock


\bibitem[\protect\citeauthoryear{{Corley}, {Lois}, and {Quezada}}{{Corley}
  et~al\mbox{.}}{2015}]%
        {Corley2015}
\bibfield{author}{\bibinfo{person}{C.~S. {Corley}}, \bibinfo{person}{F.
  {Lois}}, {and} \bibinfo{person}{S. {Quezada}}.}
  \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Web usage patterns of developers}. In
  \bibinfo{booktitle}{\emph{2015 IEEE International Conference on Software
  Maintenance and Evolution (ICSME)}}. \bibinfo{pages}{381--390}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/ICSM.2015.7332489}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Durieux, Abreu, Monperrus, and
  Bissyand{\'{e}}}{Durieux et~al\mbox{.}}{2019}]%
        {Durieux2019}
\bibfield{author}{\bibinfo{person}{Thomas Durieux}, \bibinfo{person}{Rui
  Abreu}, \bibinfo{person}{Martin Monperrus}, {and}
  \bibinfo{person}{Tegawend{\'{e}}~F. Bissyand{\'{e}}}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Interviewing the Most Successful Bot on GitHub: Dr
  Travis {CI} on 35+ Million of its Jobs}.
\newblock \bibinfo{journal}{\emph{CoRR}}  \bibinfo{volume}{abs/1904.09416}
  (\bibinfo{year}{2019}).
\newblock
\urldef\tempurl%
\url{http://arxiv.org/abs/1904.09416}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Fayolle, Moreau, Raymond, Gravier, and
  Gros}{Fayolle et~al\mbox{.}}{2010}]%
        {fayolle2010crf}
\bibfield{author}{\bibinfo{person}{Julien Fayolle}, \bibinfo{person}{Fabienne
  Moreau}, \bibinfo{person}{Christian Raymond}, \bibinfo{person}{Guillaume
  Gravier}, {and} \bibinfo{person}{Patrick Gros}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{CRF-based combination of contextual features to
  improve a posteriori word-level confidence measures}. In
  \bibinfo{booktitle}{\emph{Eleventh Annual Conference of the International
  Speech Communication Association}}.
\newblock


\bibitem[\protect\citeauthoryear{Fox, Karnawat, Mydland, Dumais, and White}{Fox
  et~al\mbox{.}}{2005}]%
        {Fox2005}
\bibfield{author}{\bibinfo{person}{Steve Fox}, \bibinfo{person}{Kuldeep
  Karnawat}, \bibinfo{person}{Mark Mydland}, \bibinfo{person}{Susan Dumais},
  {and} \bibinfo{person}{Thomas White}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{Evaluating Implicit Measures to Improve Web
  Search}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Inf. Syst.}} \bibinfo{volume}{23},
  \bibinfo{number}{2} (\bibinfo{date}{April} \bibinfo{year}{2005}).
\newblock


\bibitem[\protect\citeauthoryear{Friedman, Hastie, and Tibshirani}{Friedman
  et~al\mbox{.}}{2010}]%
        {l1l2}
\bibfield{author}{\bibinfo{person}{Jerome Friedman}, \bibinfo{person}{Trevor
  Hastie}, {and} \bibinfo{person}{Rob Tibshirani}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Regularization paths for generalized linear models
  via coordinate descent}.
\newblock \bibinfo{journal}{\emph{Journal of statistical software}}
  \bibinfo{volume}{33}, \bibinfo{number}{1} (\bibinfo{year}{2010}),
  \bibinfo{pages}{1}.
\newblock


\bibitem[\protect\citeauthoryear{gdpr.eu}{gdpr.eu}{2019}]%
        {gdpr}
\bibfield{author}{\bibinfo{person}{gdpr.eu}.} \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{{General Data Protection Regulation}}.
\newblock \bibinfo{howpublished}{\url{https://gdpr-info.eu/}}.
\newblock


\bibitem[\protect\citeauthoryear{Haiduc, Bavota, Marcus, Oliveto, De~Lucia, and
  Menzies}{Haiduc et~al\mbox{.}}{2013}]%
        {Haiduc2013}
\bibfield{author}{\bibinfo{person}{Sonia Haiduc}, \bibinfo{person}{Gabriele
  Bavota}, \bibinfo{person}{Andrian Marcus}, \bibinfo{person}{Rocco Oliveto},
  \bibinfo{person}{Andrea De~Lucia}, {and} \bibinfo{person}{Tim Menzies}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Automatic Query Reformulations for Text Retrieval
  in Software Engineering}. In \bibinfo{booktitle}{\emph{Proceedings of the
  2013 International Conference on Software Engineering}} (San Francisco, CA,
  USA) \emph{(\bibinfo{series}{ICSE '13})}. \bibinfo{publisher}{IEEE Press},
  \bibinfo{address}{Piscataway, NJ, USA}, \bibinfo{pages}{842--851}.
\newblock
\showISBNx{978-1-4673-3076-3}
\urldef\tempurl%
\url{http://dl.acm.org/citation.cfm?id=2486788.2486898}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Hassan, Jones, and Klinkner}{Hassan
  et~al\mbox{.}}{2010}]%
        {Hassan:2010:BDU:1718487.1718515}
\bibfield{author}{\bibinfo{person}{Ahmed Hassan}, \bibinfo{person}{Rosie
  Jones}, {and} \bibinfo{person}{Kristina~Lisa Klinkner}.}
  \bibinfo{year}{2010}\natexlab{}.
\newblock \showarticletitle{Beyond DCG: User Behavior As a Predictor of a
  Successful Search}. In \bibinfo{booktitle}{\emph{Proceedings of the Third ACM
  International Conference on Web Search and Data Mining}} (New York, New York,
  USA) \emph{(\bibinfo{series}{WSDM '10})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{221--230}.
\newblock
\showISBNx{978-1-60558-889-6}
\urldef\tempurl%
\url{https://doi.org/10.1145/1718487.1718515}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{{Hassan} and {Xiaoyin Wang}}{{Hassan} and
  {Xiaoyin Wang}}{2017}]%
        {foyzul2017}
\bibfield{author}{\bibinfo{person}{F. {Hassan}} {and} \bibinfo{person}{{Xiaoyin
  Wang}}.} \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Mining Readme Files to Support Automatic Building
  of Java Projects in Software Repositories}. In \bibinfo{booktitle}{\emph{2017
  IEEE/ACM 39th International Conference on Software Engineering Companion
  (ICSE-C)}}. \bibinfo{pages}{277--279}.
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1109/ICSE-C.2017.114}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Hassan~Awadallah, Fahmy, and
  Hassan~Awadalla}{Hassan~Awadallah et~al\mbox{.}}{2007}]%
        {hassanawadallah2007improving}
\bibfield{author}{\bibinfo{person}{Ahmed Hassan~Awadallah},
  \bibinfo{person}{Haytham Fahmy}, {and} \bibinfo{person}{Hany
  Hassan~Awadalla}.} \bibinfo{year}{2007}\natexlab{}.
\newblock \bibinfo{title}{Improving Named Entity Translation by Exploiting
  Comparable and Parallel Corpora}.
\newblock
\newblock
\urldef\tempurl%
\url{https://www.microsoft.com/en-us/research/publication/improving-named-entity-translation-exploiting-comparable-parallel-corpora/}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Holmes, Walker, and Murphy}{Holmes
  et~al\mbox{.}}{2005}]%
        {Holmes2005}
\bibfield{author}{\bibinfo{person}{Reid Holmes}, \bibinfo{person}{Robert~J.
  Walker}, {and} \bibinfo{person}{Gail~C. Murphy}.}
  \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{Strathcona Example Recommendation Tool}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 10th European Software
  Engineering Conference Held Jointly with 13th ACM SIGSOFT International
  Symposium on Foundations of Software Engineering}} (Lisbon, Portugal)
  \emph{(\bibinfo{series}{ESEC/FSE-13})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{237--240}.
\newblock
\showISBNx{1-59593-014-0}
\urldef\tempurl%
\url{https://doi.org/10.1145/1081706.1081744}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Hu, Zhang, Chen, Wang, and Yang}{Hu
  et~al\mbox{.}}{2011}]%
        {Hu2011}
\bibfield{author}{\bibinfo{person}{Botao Hu}, \bibinfo{person}{Yuchen Zhang},
  \bibinfo{person}{Weizhu Chen}, \bibinfo{person}{Gang Wang}, {and}
  \bibinfo{person}{Qiang Yang}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Characterizing Search Intent Diversity into Click
  Models}. In \bibinfo{booktitle}{\emph{Proceedings of the 20th International
  Conference on World Wide Web}} (Hyderabad, India) \emph{(\bibinfo{series}{WWW
  '11})}. \bibinfo{publisher}{ACM}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{17--26}.
\newblock
\showISBNx{978-1-4503-0632-4}
\urldef\tempurl%
\url{https://doi.org/10.1145/1963405.1963412}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Jhaver, Cranshaw, and Counts}{Jhaver
  et~al\mbox{.}}{2019}]%
        {jhaver2019measuring}
\bibfield{author}{\bibinfo{person}{Shagun Jhaver}, \bibinfo{person}{Justin
  Cranshaw}, {and} \bibinfo{person}{Scott Counts}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Measuring Professional Skill Development in US
  Cities Using Internet Search Queries}. In
  \bibinfo{booktitle}{\emph{Proceedings of the International AAAI Conference on
  Web and Social Media}}, Vol.~\bibinfo{volume}{13}. \bibinfo{pages}{267--277}.
\newblock


\bibitem[\protect\citeauthoryear{{Jia}, {Li}, {Yu}, {Liao}, {Wang}, {Liu}, and
  {Liu}}{{Jia} et~al\mbox{.}}{2019}]%
        {ZJia2019}
\bibfield{author}{\bibinfo{person}{Z. {Jia}}, \bibinfo{person}{S. {Li}},
  \bibinfo{person}{T. {Yu}}, \bibinfo{person}{X. {Liao}}, \bibinfo{person}{J.
  {Wang}}, \bibinfo{person}{X. {Liu}}, {and} \bibinfo{person}{Y. {Liu}}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \showarticletitle{Detecting Error-Handling Bugs without Error
  Specification Input}. In \bibinfo{booktitle}{\emph{2019 34th IEEE/ACM
  International Conference on Automated Software Engineering (ASE)}}.
  \bibinfo{pages}{213--225}.
\newblock


\bibitem[\protect\citeauthoryear{Jiang, Hassan~Awadallah, Shi, and White}{Jiang
  et~al\mbox{.}}{2015}]%
        {Jiang2015}
\bibfield{author}{\bibinfo{person}{Jiepu Jiang}, \bibinfo{person}{Ahmed
  Hassan~Awadallah}, \bibinfo{person}{Xiaolin Shi}, {and}
  \bibinfo{person}{Ryen~W. White}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{Understanding and Predicting Graded Search
  Satisfaction}. In \bibinfo{booktitle}{\emph{Proceedings of the Eighth ACM
  International Conference on Web Search and Data Mining}} (Shanghai, China)
  \emph{(\bibinfo{series}{WSDM '15})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{57--66}.
\newblock
\showISBNx{978-1-4503-3317-7}
\urldef\tempurl%
\url{https://doi.org/10.1145/2684822.2685319}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Jonnalagadda, Cohen, Wu, Liu, and
  Gonzalez}{Jonnalagadda et~al\mbox{.}}{2013}]%
        {jonnalagadda2013using}
\bibfield{author}{\bibinfo{person}{Siddhartha Jonnalagadda},
  \bibinfo{person}{Trevor Cohen}, \bibinfo{person}{Stephen Wu},
  \bibinfo{person}{Hongfang Liu}, {and} \bibinfo{person}{Graciela Gonzalez}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{Using empirically constructed lexical resources for
  named entity recognition}.
\newblock \bibinfo{journal}{\emph{Biomedical informatics insights}}
  \bibinfo{volume}{6} (\bibinfo{year}{2013}), \bibinfo{pages}{BII--S11664}.
\newblock


\bibitem[\protect\citeauthoryear{Kim, Kim, Bissyand\'{e}, Choi, Li, Klein, and
  Traon}{Kim et~al\mbox{.}}{2018}]%
        {Kim2018}
\bibfield{author}{\bibinfo{person}{Kisub Kim}, \bibinfo{person}{Dongsun Kim},
  \bibinfo{person}{Tegawend\'{e}~F. Bissyand\'{e}}, \bibinfo{person}{Eunjong
  Choi}, \bibinfo{person}{Li Li}, \bibinfo{person}{Jacques Klein}, {and}
  \bibinfo{person}{Yves~Le Traon}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{FaCoY: A Code-to-Code Search Engine}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 40th International Conference on
  Software Engineering}} (Gothenburg, Sweden) \emph{(\bibinfo{series}{ICSE
  ’18})}. \bibinfo{publisher}{Association for Computing Machinery},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{946–957}.
\newblock
\showISBNx{9781450356381}
\urldef\tempurl%
\url{https://doi.org/10.1145/3180155.3180187}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Lafferty, McCallum, and Pereira}{Lafferty
  et~al\mbox{.}}{2001}]%
        {Lafferty2001}
\bibfield{author}{\bibinfo{person}{John~D. Lafferty}, \bibinfo{person}{Andrew
  McCallum}, {and} \bibinfo{person}{Fernando C.~N. Pereira}.}
  \bibinfo{year}{2001}\natexlab{}.
\newblock \showarticletitle{Conditional Random Fields: Probabilistic Models for
  Segmenting and Labeling Sequence Data}. In
  \bibinfo{booktitle}{\emph{Proceedings of the Eighteenth International
  Conference on Machine Learning}} \emph{(\bibinfo{series}{ICML '01})}.
  \bibinfo{publisher}{Morgan Kaufmann Publishers Inc.}, \bibinfo{address}{San
  Francisco, CA, USA}, \bibinfo{pages}{282--289}.
\newblock
\showISBNx{1-55860-778-1}
\urldef\tempurl%
\url{http://dl.acm.org/citation.cfm?id=645530.655813}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Liu, Liu, and Yan}{Liu et~al\mbox{.}}{2018}]%
        {Liu2018}
\bibfield{author}{\bibinfo{person}{Chang Liu}, \bibinfo{person}{Jingjing Liu},
  {and} \bibinfo{person}{Zengwang Yan}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Personalizing Information Retrieval Using Search
  Behaviors and Time Constraints}. In \bibinfo{booktitle}{\emph{Proceedings of
  the 2018 Conference on Human Information Interaction and Retrieval}} (New
  Brunswick, NJ, USA) \emph{(\bibinfo{series}{CHIIR ’18})}.
  \bibinfo{publisher}{Association for Computing Machinery},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{261–264}.
\newblock
\showISBNx{9781450349253}
\urldef\tempurl%
\url{https://doi.org/10.1145/3176349.3176878}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Liu and Nocedal}{Liu and Nocedal}{1989}]%
        {lbgs1989}
\bibfield{author}{\bibinfo{person}{Dong~C. Liu} {and} \bibinfo{person}{Jorge
  Nocedal}.} \bibinfo{year}{1989}\natexlab{}.
\newblock \showarticletitle{On the Limited Memory BFGS Method for Large Scale
  Optimization}.
\newblock \bibinfo{journal}{\emph{Math. Program.}} \bibinfo{volume}{45},
  \bibinfo{number}{1-3} (\bibinfo{date}{Aug.} \bibinfo{year}{1989}),
  \bibinfo{pages}{503--528}.
\newblock
\showISSN{0025-5610}
\urldef\tempurl%
\url{http://dl.acm.org/citation.cfm?id=3112655.3112866}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Liu, Zhang, Wei, and Zhou}{Liu
  et~al\mbox{.}}{2011}]%
        {Liu2011}
\bibfield{author}{\bibinfo{person}{Xiaohua Liu}, \bibinfo{person}{Shaodian
  Zhang}, \bibinfo{person}{Furu Wei}, {and} \bibinfo{person}{Ming Zhou}.}
  \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{Recognizing Named Entities in Tweets}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 49th Annual Meeting of the
  Association for Computational Linguistics: Human Language Technologies -
  Volume 1}} (Portland, Oregon) \emph{(\bibinfo{series}{HLT '11})}.
  \bibinfo{publisher}{Association for Computational Linguistics},
  \bibinfo{address}{Stroudsburg, PA, USA}, \bibinfo{pages}{359--367}.
\newblock
\showISBNx{978-1-932432-87-9}
\urldef\tempurl%
\url{http://dl.acm.org/citation.cfm?id=2002472.2002519}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Lu, Zhang, and Ma}{Lu et~al\mbox{.}}{2018}]%
        {Lu18}
\bibfield{author}{\bibinfo{person}{Hongyu Lu}, \bibinfo{person}{Min Zhang},
  {and} \bibinfo{person}{Shaoping Ma}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Between Clicks and Satisfaction: Study on
  Multi-Phase User Preferences and Satisfaction for Online News Reading}. In
  \bibinfo{booktitle}{\emph{The 41st International ACM SIGIR Conference on
  Research and Development in Information Retrieval}} (Ann Arbor, MI, USA)
  \emph{(\bibinfo{series}{SIGIR ’18})}. \bibinfo{publisher}{Association for
  Computing Machinery}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{435–444}.
\newblock
\showISBNx{9781450356572}
\urldef\tempurl%
\url{https://doi.org/10.1145/3209978.3210007}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Luo, Zhang, Li, Liu, Zhang, Ma, and Yang}{Luo
  et~al\mbox{.}}{2016}]%
        {Luo16}
\bibfield{author}{\bibinfo{person}{Cheng Luo}, \bibinfo{person}{Fan Zhang},
  \bibinfo{person}{Xue Li}, \bibinfo{person}{Yiqun Liu}, \bibinfo{person}{Min
  Zhang}, \bibinfo{person}{Shaoping Ma}, {and} \bibinfo{person}{Delin Yang}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Manipulating Time Perception of Web Search Users}.
  In \bibinfo{booktitle}{\emph{Proceedings of the 2016 ACM on Conference on
  Human Information Interaction and Retrieval}} (Carrboro, North Carolina, USA)
  \emph{(\bibinfo{series}{CHIIR ’16})}. \bibinfo{publisher}{Association for
  Computing Machinery}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{293–296}.
\newblock
\showISBNx{9781450337519}
\urldef\tempurl%
\url{https://doi.org/10.1145/2854946.2854994}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Ma and Hovy}{Ma and Hovy}{2016}]%
        {ma2016end}
\bibfield{author}{\bibinfo{person}{Xuezhe Ma} {and} \bibinfo{person}{Eduard
  Hovy}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{End-to-end sequence labeling via bi-directional
  lstm-cnns-crf}.
\newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:1603.01354}}
  (\bibinfo{year}{2016}).
\newblock


\bibitem[\protect\citeauthoryear{Mao, Liu, Zhou, Nie, Song, Zhang, Ma, Sun, and
  Luo}{Mao et~al\mbox{.}}{2016}]%
        {Mao2016}
\bibfield{author}{\bibinfo{person}{Jiaxin Mao}, \bibinfo{person}{Yiqun Liu},
  \bibinfo{person}{Ke Zhou}, \bibinfo{person}{Jian-Yun Nie},
  \bibinfo{person}{Jingtao Song}, \bibinfo{person}{Min Zhang},
  \bibinfo{person}{Shaoping Ma}, \bibinfo{person}{Jiashen Sun}, {and}
  \bibinfo{person}{Hengliang Luo}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{When Does Relevance Mean Usefulness and User
  Satisfaction in Web Search?}. In \bibinfo{booktitle}{\emph{Proceedings of the
  39th International ACM SIGIR Conference on Research and Development in
  Information Retrieval}} (Pisa, Italy) \emph{(\bibinfo{series}{SIGIR ’16})}.
  \bibinfo{publisher}{Association for Computing Machinery},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{463–472}.
\newblock
\showISBNx{9781450340694}
\urldef\tempurl%
\url{https://doi.org/10.1145/2911451.2911507}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Martie, Hoek, and Kwak}{Martie
  et~al\mbox{.}}{2017}]%
        {Martie2017}
\bibfield{author}{\bibinfo{person}{Lee Martie}, \bibinfo{person}{Andr{\'e}
  van~der Hoek}, {and} \bibinfo{person}{Thomas Kwak}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Understanding the Impact of Support for Iteration
  on Code Search}. In \bibinfo{booktitle}{\emph{Proceedings of the 2017 11th
  Joint Meeting on Foundations of Software Engineering}} (Paderborn, Germany)
  \emph{(\bibinfo{series}{ESEC/FSE 2017})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{774--785}.
\newblock
\showISBNx{978-1-4503-5105-8}
\urldef\tempurl%
\url{https://doi.org/10.1145/3106237.3106293}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Mehrotra, Anderson, Diaz, Sharma, Wallach, and
  Yilmaz}{Mehrotra et~al\mbox{.}}{2017}]%
        {Mehrotra2017}
\bibfield{author}{\bibinfo{person}{Rishabh Mehrotra}, \bibinfo{person}{Ashton
  Anderson}, \bibinfo{person}{Fernando Diaz}, \bibinfo{person}{Amit Sharma},
  \bibinfo{person}{Hanna Wallach}, {and} \bibinfo{person}{Emine Yilmaz}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Auditing Search Engines for Differential
  Satisfaction Across Demographics}. In \bibinfo{booktitle}{\emph{Proceedings
  of the 26th International Conference on World Wide Web Companion}}
  \emph{(\bibinfo{series}{WWW '17 Companion})}.
\newblock


\bibitem[\protect\citeauthoryear{Meng, Nagy, Yao, Zhuang, and Argoty}{Meng
  et~al\mbox{.}}{2018}]%
        {Meng2018}
\bibfield{author}{\bibinfo{person}{Na Meng}, \bibinfo{person}{Stefan Nagy},
  \bibinfo{person}{Danfeng~(Daphne) Yao}, \bibinfo{person}{Wenjie Zhuang},
  {and} \bibinfo{person}{Gustavo~Arango Argoty}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Secure Coding Practices in Java: Challenges and
  Vulnerabilities}. In \bibinfo{booktitle}{\emph{Proceedings of the 40th
  International Conference on Software Engineering}} (Gothenburg, Sweden)
  \emph{(\bibinfo{series}{ICSE ’18})}. \bibinfo{publisher}{Association for
  Computing Machinery}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{372–383}.
\newblock
\showISBNx{9781450356381}
\urldef\tempurl%
\url{https://doi.org/10.1145/3180155.3180201}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Middleton and Krivcovs}{Middleton and
  Krivcovs}{2016}]%
        {Middleton2016}
\bibfield{author}{\bibinfo{person}{Stuart~E. Middleton} {and}
  \bibinfo{person}{Vadims Krivcovs}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Geoparsing and Geosemantics for Social Media:
  Spatiotemporal Grounding of Content Propagating Rumors to Support Trust and
  Veracity Analysis During Breaking News}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Inf. Syst.}} \bibinfo{volume}{34},
  \bibinfo{number}{3}, Article \bibinfo{articleno}{16} (\bibinfo{date}{April}
  \bibinfo{year}{2016}), \bibinfo{numpages}{26}~pages.
\newblock
\showISSN{1046-8188}
\urldef\tempurl%
\url{https://doi.org/10.1145/2842604}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Mozilla.org}{Mozilla.org}{2019}]%
        {AcceptLanguage-HTTP}
\bibfield{author}{\bibinfo{person}{Mozilla.org}.}
  \bibinfo{year}{2019}\natexlab{}.
\newblock \bibinfo{title}{{Accept-Language HTTP}}.
\newblock
  \bibinfo{howpublished}{\url{https://developer.mozilla.org/en-US/docs/Web/HTTP/Headers/Accept-Language}}.
\newblock


\bibitem[\protect\citeauthoryear{{Nanz} and {Furia}}{{Nanz} and
  {Furia}}{2015}]%
        {Nanz2015}
\bibfield{author}{\bibinfo{person}{S. {Nanz}} {and} \bibinfo{person}{C.~A.
  {Furia}}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{A Comparative Study of Programming Languages in
  Rosetta Code}. In \bibinfo{booktitle}{\emph{2015 IEEE/ACM 37th IEEE
  International Conference on Software Engineering}}, Vol.~\bibinfo{volume}{1}.
  \bibinfo{pages}{778--788}.
\newblock
\showISSN{0270-5257}
\urldef\tempurl%
\url{https://doi.org/10.1109/ICSE.2015.90}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Nasehi, Sillito, Maurer, and Burns}{Nasehi
  et~al\mbox{.}}{2012}]%
        {nasehi2012makes}
\bibfield{author}{\bibinfo{person}{Seyed~Mehdi Nasehi},
  \bibinfo{person}{Jonathan Sillito}, \bibinfo{person}{Frank Maurer}, {and}
  \bibinfo{person}{Chris Burns}.} \bibinfo{year}{2012}\natexlab{}.
\newblock \showarticletitle{What makes a good code example?: A study of
  programming Q\&A in StackOverflow}. In \bibinfo{booktitle}{\emph{2012 28th
  IEEE International Conference on Software Maintenance (ICSM)}}. IEEE,
  \bibinfo{pages}{25--34}.
\newblock


\bibitem[\protect\citeauthoryear{{Nguyen}, {Rigby}, {Nguyen}, {Palani},
  {Karanfil}, and {Nguyen}}{{Nguyen} et~al\mbox{.}}{2018}]%
        {Nguyen2018}
\bibfield{author}{\bibinfo{person}{A.~T. {Nguyen}}, \bibinfo{person}{P.~C.
  {Rigby}}, \bibinfo{person}{T. {Nguyen}}, \bibinfo{person}{D. {Palani}},
  \bibinfo{person}{M. {Karanfil}}, {and} \bibinfo{person}{T.~N. {Nguyen}}.}
  \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Statistical Translation of English Texts to API
  Code Templates}. In \bibinfo{booktitle}{\emph{2018 IEEE International
  Conference on Software Maintenance and Evolution (ICSME)}}.
  \bibinfo{pages}{194--205}.
\newblock
\showISSN{2576-3148}
\urldef\tempurl%
\url{https://doi.org/10.1109/ICSME.2018.00029}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Okazaki}{Okazaki}{2007}]%
        {CRFsuite}
\bibfield{author}{\bibinfo{person}{Naoaki Okazaki}.}
  \bibinfo{year}{2007}\natexlab{}.
\newblock \bibinfo{title}{CRFsuite: a fast implementation of Conditional Random
  Fields (CRFs)}.
\newblock
\newblock
\urldef\tempurl%
\url{http://www.chokkan.org/software/crfsuite/}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Ong, J\"{a}rvelin, Sanderson, and Scholer}{Ong
  et~al\mbox{.}}{2017}]%
        {oj17-sigir}
\bibfield{author}{\bibinfo{person}{K. Ong}, \bibinfo{person}{K. J\"{a}rvelin},
  \bibinfo{person}{M. Sanderson}, {and} \bibinfo{person}{F. Scholer}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{Using Information Scent to Understand Mobile and
  Desktop Web Search Behavior}. \bibinfo{pages}{295--304}.
\newblock


\bibitem[\protect\citeauthoryear{Paparrizos, White, and Horvitz}{Paparrizos
  et~al\mbox{.}}{2016}]%
        {paparrizos2016detecting}
\bibfield{author}{\bibinfo{person}{John Paparrizos}, \bibinfo{person}{Ryen~W
  White}, {and} \bibinfo{person}{Eric Horvitz}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Detecting devastating diseases in search logs}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 22nd ACM SIGKDD International
  Conference on Knowledge Discovery and Data Mining}}. ACM,
  \bibinfo{pages}{559--568}.
\newblock


\bibitem[\protect\citeauthoryear{Rabiner}{Rabiner}{1990}]%
        {Rabiner1990}
\bibfield{author}{\bibinfo{person}{Lawrence~R. Rabiner}.}
  \bibinfo{year}{1990}\natexlab{}.
\newblock \showarticletitle{Readings in Speech Recognition}.
\newblock \bibinfo{publisher}{Morgan Kaufmann Publishers Inc.},
  \bibinfo{address}{San Francisco, CA, USA}, Chapter A Tutorial on Hidden
  Markov Models and Selected Applications in Speech Recognition,
  \bibinfo{pages}{267--296}.
\newblock
\showISBNx{1-55860-124-4}
\urldef\tempurl%
\url{http://dl.acm.org/citation.cfm?id=108235.108253}
\showURL{%
\tempurl}


\bibitem[\protect\citeauthoryear{Radlinski and Joachims}{Radlinski and
  Joachims}{2005}]%
        {radlinski2005query}
\bibfield{author}{\bibinfo{person}{Filip Radlinski} {and}
  \bibinfo{person}{Thorsten Joachims}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{Query chains: learning to rank from implicit
  feedback}. In \bibinfo{booktitle}{\emph{Proceedings of the eleventh ACM
  SIGKDD international conference on Knowledge discovery in data mining}}. ACM,
  \bibinfo{pages}{239--248}.
\newblock


\bibitem[\protect\citeauthoryear{Rahman, Barson, Paul, Kayani, Lois, Quezada,
  Parnin, Stolee, and Ray}{Rahman et~al\mbox{.}}{2018}]%
        {Rahman:2018:EDU:3196398.3196425}
\bibfield{author}{\bibinfo{person}{Md~Masudur Rahman}, \bibinfo{person}{Jed
  Barson}, \bibinfo{person}{Sydney Paul}, \bibinfo{person}{Joshua Kayani},
  \bibinfo{person}{Federico~Andr{\'e}s Lois},
  \bibinfo{person}{Sebasti\'{a}n~Fernandez Quezada},
  \bibinfo{person}{Christopher Parnin}, \bibinfo{person}{Kathryn~T. Stolee},
  {and} \bibinfo{person}{Baishakhi Ray}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Evaluating How Developers Use General-purpose
  Web-search for Code Retrieval}. In \bibinfo{booktitle}{\emph{Proceedings of
  the 15th International Conference on Mining Software Repositories}}
  (Gothenburg, Sweden) \emph{(\bibinfo{series}{MSR '18})}.
  \bibinfo{publisher}{ACM}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{465--475}.
\newblock
\showISBNx{978-1-4503-5716-6}
\urldef\tempurl%
\url{https://doi.org/10.1145/3196398.3196425}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Rao, Bansal, Mukherjee, and Maddila}{Rao
  et~al\mbox{.}}{2020}]%
        {rao2020product}
\bibfield{author}{\bibinfo{person}{Nikitha Rao}, \bibinfo{person}{Chetan
  Bansal}, \bibinfo{person}{Subhabrata Mukherjee}, {and}
  \bibinfo{person}{Chandra Maddila}.} \bibinfo{year}{2020}\natexlab{}.
\newblock \bibinfo{title}{Product Insights: Analyzing Product Intents in Web
  Search}.
\newblock
\newblock
\showeprint[arxiv]{2005.08591}~[cs.IR]


\bibitem[\protect\citeauthoryear{Rastogi, Nagappan, Gousios, and van~der
  Hoek}{Rastogi et~al\mbox{.}}{2018}]%
        {Rastogi2018}
\bibfield{author}{\bibinfo{person}{Ayushi Rastogi}, \bibinfo{person}{Nachiappan
  Nagappan}, \bibinfo{person}{Georgios Gousios}, {and}
  \bibinfo{person}{Andr\'{e} van~der Hoek}.} \bibinfo{year}{2018}\natexlab{}.
\newblock \showarticletitle{Relationship between Geographical Location and
  Evaluation of Developer Contributions in Github}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 12th ACM/IEEE International
  Symposium on Empirical Software Engineering and Measurement}} (Oulu, Finland)
  \emph{(\bibinfo{series}{ESEM ’18})}. \bibinfo{publisher}{Association for
  Computing Machinery}, \bibinfo{address}{New York, NY, USA}, Article
  \bibinfo{articleno}{22}, \bibinfo{numpages}{8}~pages.
\newblock
\showISBNx{9781450358231}
\urldef\tempurl%
\url{https://doi.org/10.1145/3239235.3240504}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Roth and Yih}{Roth and Yih}{2005}]%
        {Roth2005}
\bibfield{author}{\bibinfo{person}{Dan Roth} {and} \bibinfo{person}{Wen-tau
  Yih}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{Integer Linear Programming Inference for
  Conditional Random Fields}. In \bibinfo{booktitle}{\emph{Proceedings of the
  22Nd International Conference on Machine Learning}} (Bonn, Germany)
  \emph{(\bibinfo{series}{ICML '05})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{736--743}.
\newblock
\showISBNx{1-59593-180-5}
\urldef\tempurl%
\url{https://doi.org/10.1145/1102351.1102444}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Sadowski, Stolee, and Elbaum}{Sadowski
  et~al\mbox{.}}{2015}]%
        {Sadowski2015}
\bibfield{author}{\bibinfo{person}{Caitlin Sadowski},
  \bibinfo{person}{Kathryn~T. Stolee}, {and} \bibinfo{person}{Sebastian
  Elbaum}.} \bibinfo{year}{2015}\natexlab{}.
\newblock \showarticletitle{How Developers Search for Code: A Case Study}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2015 10th Joint Meeting on
  Foundations of Software Engineering}} (Bergamo, Italy)
  \emph{(\bibinfo{series}{ESEC/FSE 2015})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{191--201}.
\newblock
\showISBNx{978-1-4503-3675-8}
\urldef\tempurl%
\url{https://doi.org/10.1145/2786805.2786855}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Sena, Coelho, Kulesza, and Bonif\'{a}cio}{Sena
  et~al\mbox{.}}{2016}]%
        {SenaMSR16}
\bibfield{author}{\bibinfo{person}{Dem\'{o}stenes Sena},
  \bibinfo{person}{Roberta Coelho}, \bibinfo{person}{Uir\'{a} Kulesza}, {and}
  \bibinfo{person}{Rodrigo Bonif\'{a}cio}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Understanding the Exception Handling Strategies of
  Java Libraries: An Empirical Study}. In \bibinfo{booktitle}{\emph{Proceedings
  of the 13th International Conference on Mining Software Repositories}}
  (Austin, Texas) \emph{(\bibinfo{series}{MSR ’16})}.
  \bibinfo{publisher}{Association for Computing Machinery},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{212–222}.
\newblock
\showISBNx{9781450341868}
\urldef\tempurl%
\url{https://doi.org/10.1145/2901739.2901757}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Shokouhi, Ozertem, and Craswell}{Shokouhi
  et~al\mbox{.}}{2016}]%
        {Shokouhi2016}
\bibfield{author}{\bibinfo{person}{Milad Shokouhi}, \bibinfo{person}{Umut
  Ozertem}, {and} \bibinfo{person}{Nick Craswell}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Did You Say U2 or YouTube?: Inferring Implicit
  Transcripts from Voice Search Logs} \emph{(\bibinfo{series}{WWW '16})}.
  \bibinfo{pages}{1215--1224}.
\newblock
\showISBNx{978-1-4503-4143-1}
\urldef\tempurl%
\url{https://doi.org/10.1145/2872427.2882994}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Sim, Umarji, Ratanotayanon, and Lopes}{Sim
  et~al\mbox{.}}{2011}]%
        {Sim2011}
\bibfield{author}{\bibinfo{person}{Susan~Elliott Sim}, \bibinfo{person}{Medha
  Umarji}, \bibinfo{person}{Sukanya Ratanotayanon}, {and}
  \bibinfo{person}{Cristina~V. Lopes}.} \bibinfo{year}{2011}\natexlab{}.
\newblock \showarticletitle{How Well Do Search Engines Support Code Retrieval
  on the Web?}
\newblock \bibinfo{journal}{\emph{ACM Trans. Softw. Eng. Methodol.}}
  \bibinfo{volume}{21}, \bibinfo{number}{1}, Article \bibinfo{articleno}{4}
  (\bibinfo{date}{Dec.} \bibinfo{year}{2011}), \bibinfo{numpages}{25}~pages.
\newblock
\showISSN{1049-331X}
\urldef\tempurl%
\url{https://doi.org/10.1145/2063239.2063243}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Sindhgatta}{Sindhgatta}{2006}]%
        {Sindhgatta2006}
\bibfield{author}{\bibinfo{person}{Renuka Sindhgatta}.}
  \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Using an Information Retrieval System to Retrieve
  Source Code Samples}. In \bibinfo{booktitle}{\emph{Proceedings of the 28th
  International Conference on Software Engineering}} (Shanghai, China)
  \emph{(\bibinfo{series}{ICSE '06})}. \bibinfo{publisher}{ACM},
  \bibinfo{address}{New York, NY, USA}, \bibinfo{pages}{905--908}.
\newblock
\showISBNx{1-59593-375-1}
\urldef\tempurl%
\url{https://doi.org/10.1145/1134285.1134448}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Stolee, Elbaum, and Dobos}{Stolee
  et~al\mbox{.}}{2014}]%
        {Stolee:2014:SSS:2628068.2581377}
\bibfield{author}{\bibinfo{person}{Kathryn~T. Stolee},
  \bibinfo{person}{Sebastian Elbaum}, {and} \bibinfo{person}{Daniel Dobos}.}
  \bibinfo{year}{2014}\natexlab{}.
\newblock \showarticletitle{Solving the Search for Source Code}.
\newblock \bibinfo{journal}{\emph{ACM Trans. Softw. Eng. Methodol.}}
  \bibinfo{volume}{23}, \bibinfo{number}{3}, Article \bibinfo{articleno}{26}
  (\bibinfo{date}{June} \bibinfo{year}{2014}), \bibinfo{numpages}{45}~pages.
\newblock
\showISSN{1049-331X}
\urldef\tempurl%
\url{https://doi.org/10.1145/2581377}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Stylos and Myers}{Stylos and Myers}{2006}]%
        {stylos2006mica}
\bibfield{author}{\bibinfo{person}{Jeffrey Stylos} {and}
  \bibinfo{person}{Brad~A Myers}.} \bibinfo{year}{2006}\natexlab{}.
\newblock \showarticletitle{Mica: A web-search tool for finding api components
  and examples}. In \bibinfo{booktitle}{\emph{Visual Languages and
  Human-Centric Computing (VL/HCC'06)}}. IEEE, \bibinfo{pages}{195--202}.
\newblock


\bibitem[\protect\citeauthoryear{{Vasilescu}, {Filkov}, and
  {Serebrenik}}{{Vasilescu} et~al\mbox{.}}{2013}]%
        {B_Vasilescu2013}
\bibfield{author}{\bibinfo{person}{B. {Vasilescu}}, \bibinfo{person}{V.
  {Filkov}}, {and} \bibinfo{person}{A. {Serebrenik}}.}
  \bibinfo{year}{2013}\natexlab{}.
\newblock \showarticletitle{StackOverflow and GitHub: Associations between
  Software Development and Crowdsourced Knowledge}. In
  \bibinfo{booktitle}{\emph{2013 International Conference on Social
  Computing}}. \bibinfo{pages}{188--195}.
\newblock


\bibitem[\protect\citeauthoryear{Viera and Garrett}{Viera and Garrett}{2005}]%
        {kappa}
\bibfield{author}{\bibinfo{person}{Anthony~J. Viera} {and}
  \bibinfo{person}{Joanne~M. Garrett}.} \bibinfo{year}{2005}\natexlab{}.
\newblock \showarticletitle{Understanding interobserver agreement: the kappa
  statistic.}
\newblock \bibinfo{journal}{\emph{Family Medicine}}  \bibinfo{volume}{37.5}
  (\bibinfo{year}{2005}), \bibinfo{pages}{360--363}.
\newblock


\bibitem[\protect\citeauthoryear{Wang}{Wang}{2009}]%
        {Wang09}
\bibfield{author}{\bibinfo{person}{Yefeng Wang}.}
  \bibinfo{year}{2009}\natexlab{}.
\newblock \showarticletitle{Annotating and Recognising Named Entities in
  Clinical Notes}. In \bibinfo{booktitle}{\emph{{ACL} 2009, Proceedings of the
  47th Annual Meeting of the Association for Computational Linguistics and the
  4th International Joint Conference on Natural Language Processing of the
  AFNLP, 2-7 August 2009, Singapore, Student Research Workshop}}.
  \bibinfo{pages}{18--26}.
\newblock


\bibitem[\protect\citeauthoryear{Wei, Chen, Xu, He, and Gui}{Wei
  et~al\mbox{.}}{2016}]%
        {wei2016disease}
\bibfield{author}{\bibinfo{person}{Qikang Wei}, \bibinfo{person}{Tao Chen},
  \bibinfo{person}{Ruifeng Xu}, \bibinfo{person}{Yulan He}, {and}
  \bibinfo{person}{Lin Gui}.} \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Disease named entity recognition by combining
  conditional random fields and bidirectional recurrent neural networks}.
\newblock \bibinfo{journal}{\emph{Database}}  \bibinfo{volume}{2016}
  (\bibinfo{year}{2016}).
\newblock


\bibitem[\protect\citeauthoryear{Xia, Bao, Lo, Kochhar, Hassan, and Xing}{Xia
  et~al\mbox{.}}{2017}]%
        {Xia:2017}
\bibfield{author}{\bibinfo{person}{Xin Xia}, \bibinfo{person}{Lingfeng Bao},
  \bibinfo{person}{David Lo}, \bibinfo{person}{Pavneet~Singh Kochhar},
  \bibinfo{person}{Ahmed~E. Hassan}, {and} \bibinfo{person}{Zhenchang Xing}.}
  \bibinfo{year}{2017}\natexlab{}.
\newblock \showarticletitle{What do developers search for on the web?}
\newblock \bibinfo{journal}{\emph{Empirical Software Engineering}}
  \bibinfo{volume}{22} (\bibinfo{date}{04} \bibinfo{year}{2017}).
\newblock
\urldef\tempurl%
\url{https://doi.org/10.1007/s10664-017-9514-4}
\showDOI{\tempurl}


\bibitem[\protect\citeauthoryear{Zhang, Jain, Khandelwal, Kaushik, Ge, and
  Hu}{Zhang et~al\mbox{.}}{2016}]%
        {Zhang2016}
\bibfield{author}{\bibinfo{person}{Hongyu Zhang}, \bibinfo{person}{Anuj Jain},
  \bibinfo{person}{Gaurav Khandelwal}, \bibinfo{person}{Chandrashekhar
  Kaushik}, \bibinfo{person}{Scott Ge}, {and} \bibinfo{person}{Wenxiang Hu}.}
  \bibinfo{year}{2016}\natexlab{}.
\newblock \showarticletitle{Bing Developer Assistant: Improving Developer
  Productivity by Recommending Sample Code}. In
  \bibinfo{booktitle}{\emph{Proceedings of the 2016 24th ACM SIGSOFT
  International Symposium on Foundations of Software Engineering}} (Seattle,
  WA, USA) \emph{(\bibinfo{series}{FSE 2016})}. \bibinfo{publisher}{Association
  for Computing Machinery}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{pages}{956–961}.
\newblock
\showISBNx{9781450342186}
\urldef\tempurl%
\url{https://doi.org/10.1145/2950290.2983955}
\showDOI{\tempurl}


\end{thebibliography}


==> taxonomy.tex <==
\newcommand{\query}[1]{\emph{``#1''}}

\section{Query taxonomy}
\label{sec:taxonomy}

There are many reasons why software developers search the web, for example to learn more about a technology or to debug an error message they encountered. 

To better understand the motivations behind web searches related to software technologies and to derive an initial taxonomy of search intent, we manually labelled three sets of search queries. Each dataset contained the query and the URLs that the user clicked on (if any) for 50 web searches. When needed, the raters searched for the query and considered the entire search results. In total, we labelled 150 web searches.

\begin{itemize}
    \item \textsc{TensorFlow \#1.} We randomly selected 50 web searches that included the word ``TensorFlow''. This dataset was labelled independently by two raters who followed an open coding approach, i.e., rather than predefined labels, the labels emerging during the coding of the web searches. For each web search, exactly one category was assigned. The raters then met and discussed the categories and agreed on an initial set of categories: \emph{debug, how-to, installation, learn, navigational,} and \emph{misc}.
    \item \textsc{TensorFlow \#2.} This dataset of 50 web searches for ``TensorFlow'' was used to further validated the categories and to measure inter-rater agreement. Three raters independently labeled the dataset with the categories from the previous dataset. No new categories emerged. The pairwise Cohen Kappa agreement~\cite{cohen1960coefficient} between the three raters was 0.469, 0.530, and 0.637; the Fleiss Kappa agreement~\cite{fleiss1971measuring} among all three raters was 0.545.
    \item \textsc{Xamarin.} This dataset was used to validate the categories for a different technology. The dataset included 50 web searches for ``Xamarin''. Two raters independently labelled the dataset with the categories from the previous dataset. The Cohen Kappa agreement between the two raters was 0.524. For this dataset, a new category emerged: \emph{api} for any searches related to documentation on how to use certain Xamarin APIs.
\end{itemize}	

The agreement scores indicate a moderate agreement according to the classification by Landis and Koch~\cite{landis1977measurement}. When the raters disagreed, this was either because of lack of context (\query{3559a tensorflow}, \query{tensorflow 1.13 rc0 .whl}) or for queries where multiple categoris were applicable (\query{tensorflow tools}).

The resulting taxonomy is summarized in Table~\ref{table:taxonomy} and discussed in the rest of this section.

\begin{table}
\setlength\belowcaptionskip{7pt}
 \begin{tabular}{|l|p{5.8cm}|}
 \hline
 \textbf{Intent} & \textbf{Description} \\ \hline
 Debug & Find information to debug an error or an issue  \\ \hline
 How-to & Find information to accomplish a specific SE related task \\ \hline
 Learn & Find information to learn about a SE related topic \\ \hline
 API & Navigate to information about a specific API element. \\ \hline
 Navigational & Navigate to a specific web-page on a SE related topic \\ \hline
 Installation & Install a software, tool, package, etc. \\ \hline
 Misc & None of the above intents is suitable \\ \hline
\end{tabular}
\caption{Taxonomy of SE related search queries}
\label{table:taxonomy}
\end{table}

\textbf{Debug.} This category captures web searches that are related to debugging an error or issue. Typical searches include error messages (\query{tensorflow/core/framework/op.h: No such file or directory}), parts of stack traces (\query{Java org tensorflow lite NativeInterpreterWrapper createErrorReporter}), and sometimes a description of the context of the error (\query{xamarin SIGSEGV after upgrading to visual studio 2019}), which often can be short and abstract (\query{tensorflow1.3 MKL libdl.so.2}). For this type of query, users typically often click on StackOverflow search results, the respective issue trackers, and discussions in web forums.

\textbf{How-to.} This category captures web searches that are related to accomplishing a specific task with a software technology. These queries often contain a short description of what the user wants to accomplish (\query{tensorflow get all tensors}, \query{force tensorflow to use gpus}, \query{launch canera on camra button click in xamarin forms}) and in some cases the technology they want to use (\query{RandomShuffleQueue tensorflow}). For most of these queries,  users click on StackOverflow results and when available official web forums and blogs. 

\textbf{Learn.} This category captures queries related to learning about an abstract topic related to the software. Example queries are \query{tensorflow python tutorial}, \query{tensorflow tools}, \query{tensorflow deep learning}, or \query{xamarin testing}. 

\textbf{API.} This category represents web searches where the user wants to learn more about a specific API element in the software. Searches related to specific API were much more frequent in Xamarin than in TensorFlow, hence we created a separate category. Examples are \query{xamarin.controls.signaturepad.forms} and \query{xamarin ActivityIndicator}.

\textbf{Navigational.} This category is related to queries where the search engine is used to navigate to a specific resource or web-page. Example queries are \query{TensorFlow: Large-scale machine learning on heterogeneous systems} and \query{o'reilly TensorFlow for Deep Learning}. In both cases, the user knew their destination and used the search engine as a shortcut/bookmark to get to a book or video respectively.

\textbf{Installation.} This category is for searches with the goal to install the software. Often these searches include the target environment (\query{tensorflow gpu keras 2019 windows 10}), version numbers, and simply the word download (\query{tensorflow 1.13 for windows download}). In many cases these searches end up at download or install pages on the official webpages but not always. For example, for the query \query{tensorflow gpu keras 2019 windows 10}, the user clicked on a Medium.com post that in detail describe the nine steps necessary to setup the Keras deep learning framework on Windows 10 on both GPU and CPU systems. Interestingly searches related to installation were more common in our samples for TensorFlow than for Xamarin.

% \footnote{\url{ https://medium.com/@ab9.bhatia/set-up-gpu-accelerated-tensorflow-keras-on-windows-10-with-anaconda-e71bfa9506d1 }}

\textbf{Misc.} This category was used when none of the above intents was suitable or when insufficient context was available to make a decision. An example from this category is \query{3559a tensorflow}.

%%AHA: @chetan, any thoughts on how this taxonomy could be used to help developers in or outside search engines
